The effect of sound speed on the gravitational wave spectrum of first order phase transitions in the early universe

Gravitational waves from first-order phase transitions are a promising probe of physics beyond the Standard Model, as many extensions of the standard model result in first-order phase transitions in the early universe, from which the resulting gravitational waves could be detectable with the upcoming Laser Interferometer Space Antenna (LISA). The properties of the phase transition and the resulting gravitational wave spectrum are determined by five key parameters: the nucleation temperature $T_n$, phase transition strength at the nucleation temperature $\alpha_n$, bubble wall speed $v_\text{wall}$, transition rate $\beta$ and the sound speed $c_s$. Of these, the sound speed $c_s$ is determined by the equation of state $p(T,\phi)$. In most studies, the plasma of the early universe has been assumed to be ultrarelativistic and therefore following the bag equation of state with $c_s = \frac{1}{\sqrt{3}}$. In this thesis, the PTtools simulation framework for first-order phase transitions, based on the Sound Shell Model, has been extended to include support for arbitrary equations of state and therefore for a temperature- and phase-dependent sound speed $c_s(T,\phi)$. The thesis also functions as a reference manual for PTtools. The framework has been tested with the constant sound speed model, in which the sound speed is a different constant in each phase. The sound speed has been shown to have a significant effect on the resulting gravitational wave spectrum, especially when changing the sound speed results in a change in the type of the solution. This has laid the groundwork for simulating cosmological phase transitions with realistic equations of state. This will result in in gravitational wave spectra that can be used in the LISA data analysis pipeline to search for the existence and parameters of a first-order phase transition in the early universe.

==> Makefile <==
all: clean pdf
clean:
	rm -f ./*.aux ./*.bbl ./*.bcf ./*.blg ./*.fdb_latexmk ./*.fls ./*.gz ./*.ilg ./*.ind ./*.lof ./*.log ./*.lot ./*.nlo ./*.nls ./*.out ./*.tdo ./*.toc ./*.xml \
		./tex/*.dvi ./tex/*.log ./main.pdf
pdf:
	# Allow exit code 12. The double $$ is needed in a Makefile to refer to a shell variable instead of a make variable.
	# https://stackoverflow.com/a/16315249
	latexmk  # -f || [ $$? -eq 12 ]


==> babelbst.tex <==
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tktl.dtx  (with options: `babelbst')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 2002 Mikael Puolakka.
%% 
%% This file may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either
%% version 1.2 of this license or (at your option) any later
%% version. The latest version of this license is in
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.2 or later is part of all distributions of
%% LaTeX version 1999/12/01 or later.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
%% This is file `babelbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%%
%% Copyright 1994-1999 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[1999/05/28 3.89 (PWD)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\iflanguage{finnish}{\input{finnbst}}{
  \iflanguage{english}{\input{englbst}}{
    \iflanguage{swedish}{\input{swedbst}}{
      \input{finnbst}
    }
  }
}
%%
%%
%% End of file `babelbst.tex'.
%% 
%%
%% End of file `babelbst.tex'.


==> englbst.tex <==
%%
%% This is file `englbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tktl.dtx  (with options: `englbst')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 2002 Mikael Puolakka.
%% 
%% This file may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either
%% version 1.2 of this license or (at your option) any later
%% version. The latest version of this license is in
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.2 or later is part of all distributions of
%% LaTeX version 1999/12/01 or later.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
%% This is file `englbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%%
%% Copyright 1994-1999 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[1999/05/28 3.89 (PWD)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{and}
\def\bbletal{et~al} % Piste sijoitetaan tarvittaessa per��n!
\def\bbleditors{editors}        \def\bbleds{eds.}
\def\bbleditor{editor}          \def\bbled{ed.}
\def\bbledby{edited by}
\def\bbledition{edition}        \def\bbledn{edn.}
\def\bblvolume{volume}          \def\bblvol{vol.}
\def\bblof{of}
\def\bblnumber{number}          \def\bblno{no.}
\def\bblin{in}
\def\bblpages{pages}            \def\bblpp{pp.}
\def\bblpage{page}              \def\bblp{p.}
\def\bblchapter{chapter}        \def\bblchap{chap.}
\def\bbltechreport{Technical Report}
\def\bbltechrep{Tech. Rep.}
\def\bblmthesis{Master's thesis}
\def\bblphdthesis{Ph.D. thesis}
\def\bblfirst{first}            \def\bblfirsto{1st}
\def\bblsecond{second}          \def\bblsecondo{2nd}
\def\bblthird{third}            \def\bblthirdo{3rd}
\def\bblfourth{fourth}          \def\bblfourtho{4th}
\def\bblfifth{fifth}            \def\bblfiftho{5th}
\def\bblst{st}  \def\bblnd{nd}  \def\bblrd{rd}
\def\bblth{th}
\def\bbljan{January}  \def\bblfeb{February}  \def\bblmar{March}
\def\bblapr{April}    \def\bblmay{May}       \def\bbljun{June}
\def\bbljul{July}     \def\bblaug{August}    \def\bblsep{September}
\def\bbloct{October}  \def\bblnov{November}  \def\bbldec{December}
\def\bblins{in} % Oma lis�ys: "in" series.
\def\bblinj{in} % Oma lis�ys: "in" journal.
%%
%%
%% End of file `babelbst.tex'.
%% 
%%
%% End of file `englbst.tex'.


==> fig/const_cs_gw_snr.tex <==
\begin{table}
\centering
\caption{Signal-to-noise ratios of the gravitational wave power spectra of fig \ref{fig:omgw0}}
\begin{tabular}{l|l|l|l}
Model & \multicolumn{3}{l}{$\v_\text{wall}$} \\
& 0.30 & 0.68 & 0.90
\hline \\
$c_{s,s}^2=1/3, c_{s,b}^2=1/3$ & 0.7 & 71.3 & 2.6 \\
$c_{s,s}^2=1/3, c_{s,b}^2=1/4$ & 0.2 & 3.5 & 0.3 \\
$c_{s,s}^2=1/4, c_{s,b}^2=1/3$ & 1.0 & 70.8 & 2.7 \\
$c_{s,s}^2=1/4, c_{s,b}^2=1/4$ & 0.3 & 4.3 & 0.3 \hline \\
$c_{s,s}^2=1/3, c_{s,b}^2=1/3$ & 2.8 & 218.2 & 26.1 \\
$c_{s,s}^2=1/3, c_{s,b}^2=1/4$ & 1.1 & 50.2 & 4.7 \\
$c_{s,s}^2=1/4, c_{s,b}^2=1/3$ & 3.8 & 574.4 & 26.3 \\
$c_{s,s}^2=1/4, c_{s,b}^2=1/4$ & 1.6 & 72.8 & 5.2 \\
\end{tabular}
\label{table:const_cs_gw_snr}
\end{table}


==> finnbst.tex <==
%%
%% This is file `finnbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tktl.dtx  (with options: `finnbst')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 2002 Mikael Puolakka.
%% 
%% This file may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either
%% version 1.2 of this license or (at your option) any later
%% version. The latest version of this license is in
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.2 or later is part of all distributions of
%% LaTeX version 1999/12/01 or later.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
%% This is file `finnbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%%
%% Copyright 1994-1999 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[1999/05/28 3.89 (PWD)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{ja}
\def\bbletal{et~al} % Piste sijoitetaan tarvittaessa per��n!
\def\bbleditors{toimittajat}
\def\bbleds{toim.}
\def\bbleditor{toimittaja}
\def\bbled{toim.}
\def\bbledby{toimittanut}
\def\bbledition{painos}
\def\bbledn{painos}
\def\bblvolume{osa}
\def\bblvol{osa}
\def\bblof{sarjasta}
\def\bblnumber{numero}
\def\bblno{no.}
\def\bblin{teoksessa}
\def\bblpages{sivut}
\def\bblpp{ss.}
\def\bblpage{sivu}
\def\bblp{s.}
\def\bblchapter{luku}
\def\bblchap{luku}
\def\bbltechreport{tekninen raportti}
\def\bbltechrep{tekn. rap.}
\def\bblmthesis{pro gradu}
\def\bblphdthesis{v�it�skirja}
\def\bblfirst{ensimm�inen}
\def\bblfirsto{1.}
\def\bblsecond{toinen}
\def\bblsecondo{2.}
\def\bblthird{kolmas}
\def\bblthirdo{3.}
\def\bblfourth{nelj�s}
\def\bblfourtho{4.}
\def\bblfifth{viides}
\def\bblfiftho{5.}
\def\bblst{.}
\def\bblnd{.}
\def\bblrd{.}
\def\bblth{.}
\def\bbljan{tammikuu}
\def\bblfeb{helmikuu}
\def\bblmar{maaliskuu}
\def\bblapr{huhtikuu}
\def\bblmay{toukokuu}
\def\bbljun{kes�kuu}
\def\bbljul{hein�kuu}
\def\bblaug{elokuu}
\def\bblsep{syyskuu}
\def\bbloct{lokakuu}
\def\bblnov{marraskuu}
\def\bbldec{joulukuu}
\def\bblins{sarjassa} % Oma lis�ys: "in" series.
\def\bblinj{julkaisussa} % Oma lis�ys: "in" journal.
%%
%%
%% End of file `babelbst.tex'.
%% 
%%
%% End of file `finnbst.tex'.


==> swedbst.tex <==
%%
%% This is file `swedbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% tktl.dtx  (with options: `swedbst')
%% 
%% This is a generated file.
%% 
%% Copyright (C) 2002 Mikael Puolakka.
%% 
%% This file may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either
%% version 1.2 of this license or (at your option) any later
%% version. The latest version of this license is in
%% 
%%    http://www.latex-project.org/lppl.txt
%% 
%% and version 1.2 or later is part of all distributions of
%% LaTeX version 1999/12/01 or later.
%% 
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%
%% This is file `swedbst.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% merlin.mbs  (with options: `bblbst')
%%
%% Copyright 1994-1999 Patrick W Daly
 % ===============================================================
 % IMPORTANT NOTICE:
 % This bibliographic style (bst) file has been generated from one or
 % more master bibliographic style (mbs) files, listed above.
 %
 % This generated file can be redistributed and/or modified under the terms
 % of the LaTeX Project Public License Distributed from CTAN
 % archives in directory macros/latex/base/lppl.txt; either
 % version 1 of the License, or any later version.
 % ===============================================================
 % Name and version information of the main mbs file:
 % \ProvidesFile{merlin.mbs}[1999/05/28 3.89 (PWD)]
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{och}
\def\bbletal{et.al} % Piste sijoitetaan tarvittaessa per��n!
\def\bbleditors{redakt�rer}
\def\bbleds{red.}
\def\bbleditor{redakt�r}
\def\bbled{red.}
\def\bbledby{redigerad av}
\def\bbledition{utg�va}
\def\bbledn{utg.}
\def\bblvolume{volym}
\def\bblvol{vol.}
\def\bblof{ur serien}
\def\bblnumber{nummer}
\def\bblno{nr.}
\def\bblin{i verket}
\def\bblpages{sidorna}
\def\bblpp{ss.}
\def\bblpage{sidan}
\def\bblp{s.}
\def\bblchapter{kapitel}
\def\bblchap{kap.}
\def\bbltechreport{teknisk rapport}
\def\bbltechrep{tekn.rap.}
\def\bblmthesis{pro gradu}
\def\bblphdthesis{doktorsavhandling}
\def\bblfirst{f�rsta}
\def\bblfirsto{f�rsta}
\def\bblsecond{andra}
\def\bblsecondo{andra}
\def\bblthird{tredje}
\def\bblthirdo{tredje}
\def\bblfourth{fj�rde}
\def\bblfourtho{fj�rde}
\def\bblfifth{femte}
\def\bblfiftho{femte}
\def\bblst{:a}  \def\bblnd{:a}  \def\bblrd{:e}
\def\bblth{:e}
\def\bbljan{januari}  \def\bblfeb{februari}  \def\bblmar{mars}
\def\bblapr{april}    \def\bblmay{maj}       \def\bbljun{juni}
\def\bbljul{juli}     \def\bblaug{augusti}   \def\bblsep{september}
\def\bbloct{oktober}  \def\bblnov{november}  \def\bbldec{december}
\def\bblins{i serie} % Oma lis�ys: "in" series.
\def\bblinj{i journalen} % Oma lis�ys: "in" journal.
%%
%%
%% End of file `babelbst.tex'.
%% 
%%
%% End of file `swedbst.tex'.

